Digital Platform Consolidation and Offline Expansion: Strategic Convergence and Market Welfare in China's Second-hand Real Estate Market

This study analyzes the impact of offline expansion and online platform consolidation in China's second-hand real estate market. Using micro-level transaction data and difference-in-differences estimations, we find offline store entry significantly boosts transaction volumes (9-10\%) and reduces price concessions (1\%) initially, though effects diminish over time. Platform consolidation via Lianjia's Agent Cooperation Network yields delayed yet persistent transaction volume increases (5-6\%), particularly in less concentrated markets, and consistently lowers price concessions. These strategies sustainably enhance brokerage competitiveness, bargaining power, and market welfare, despite increased market concentration, ultimately benefiting sellers and improving overall efficiency.

==> result_tables/clustering_indices.tex <==
\begin{tabular}{lllllllll}
\hline
 city      & index                    & 2016   & 2017   & 2018   & 2019   & 2020   & 2021    & 2022   \\
\hline
 Beijing   & average local clustering & 0.15   & 0.18   & 0.19   & 0.19   & 0.20   &         &        \\
 Beijing   & global clustering        & 0.30   & 0.36*  & 0.38*  & 0.38*  & 0.41*  &         &        \\
 Chengdu   & average local clustering & 0.20   & 0.21   & 0.20   & 0.22   & 0.23   &         &        \\
 Chengdu   & global clustering        & 0.29   & 0.29   & 0.33*  & 0.35*  & 0.38*  &         &        \\
 Chongqing & average local clustering & 0.09   & 0.13   & 0.14   & 0.16   & 0.21   & 0.23    & 0.24   \\
 Chongqing & global clustering        & 0.20   & 0.24   & 0.28   & 0.31*  & 0.44*  & 0.52**  & 0.56** \\
 Guangzhou & average local clustering & 0.06   & 0.16   & 0.17   & 0.16   & 0.24   & 0.27    & 0.28   \\
 Guangzhou & global clustering        & 0.12   & 0.33*  & 0.40*  & 0.31*  & 0.43*  & 0.53**  & 0.57** \\
 Hangzhou  & average local clustering & 0.14   & 0.16   & 0.16   & 0.18   & 0.25   & 0.25    & 0.24   \\
 Hangzhou  & global clustering        & 0.24   & 0.32*  & 0.35*  & 0.34*  & 0.46*  & 0.48*   & 0.51** \\
 Nanjing   & average local clustering & 0.16   & 0.23   & 0.23   & 0.23   & 0.25   & 0.25    & 0.25   \\
 Nanjing   & global clustering        & 0.29   & 0.42*  & 0.44*  & 0.43*  & 0.46*  & 0.48*   & 0.50*  \\
 Shanghai  & average local clustering & 0.21   & 0.21   & 0.20   & 0.21   & 0.19   & 0.18    & 0.18   \\
 Shanghai  & global clustering        & 0.35*  & 0.43*  & 0.43*  & 0.40*  & 0.33*  & 0.34*   & 0.39*  \\
 Shenzhen  & average local clustering & 0.14   & 0.22   & 0.21   & 0.18   & 0.25   &         &        \\
 Shenzhen  & global clustering        & 0.27   & 0.40*  & 0.40*  & 0.37*  & 0.49*  &         &        \\
 Tianjin   & average local clustering & 0.13   & 0.16   & 0.16   & 0.19   & 0.24   & 0.24    & 0.24   \\
 Tianjin   & global clustering        & 0.20   & 0.28   & 0.27   & 0.32*  & 0.43*  & 0.46*   & 0.47*  \\
 Wuhan     & average local clustering & 0.09   & 0.15   & 0.17   & 0.19   & 0.25   &         &        \\
 Wuhan     & global clustering        & 0.26   & 0.38*  & 0.44*  & 0.41*  & 0.55** &         &        \\
\hline
\end{tabular}

==> result_tables/donut_robust.tex <==
% latex table generated in R 4.2.0 by xtable 1.8-4 package
% Mon Jul  8 21:17:07 2024
\begin{table}[ht]
\centering
\caption{RD Analysis Donut RD Results with and without Controls} 
\label{tab:rd_robust_results}
\begin{tabular}{lllllllll}
  \hline
 &  & \multicolumn{3}{c}{Without Control} & \multicolumn{3}{c}{With Control} & \\
Donut Width & Method & Coef & SE & p-value & Coef & SE & p-value & Drop Ratio(\%) \\ 
  \hline
donut\_0.005 & Robust & -47449 & 24227 & 0.0502 & -80978 & 30701 & 0.00835 & 7.85 \\ 
  donut\_0.0075 & Robust & -42335 & 26685 & 0.113 & -79698 & 33726 & 0.0181 & 11.73 \\ 
  donut\_0.01 & Robust & -64934 & 30585 & 0.0337 & -90221 & 38228 & 0.0183 & 15.59 \\ 
  donut\_0.0125 & Robust & -62531 & 34437 & 0.0694 & -78610 & 43377 & 0.07 & 19.48 \\ 
  donut\_0.015 & Robust & -36788 & 39345 & 0.35 & -94673 & 50238 & 0.0595 & 23.66 \\ 
  donut\_0.0175 & Robust & 4018 & 44747 & 0.928 & -76155 & 56672 & 0.179 & 27.88 \\ 
  donut\_0.02 & Robust & 28087 & 49139 & 0.568 & -44578 & 60900 & 0.464 & 31.71 \\ 
   \hline
\end{tabular}
Note that the cutoff is 0.41, the main bandwidth is 0.066 and the bias bandwidth is 0.135.

\end{table}



==> result_tables/dynamic.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(lead times)}&\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{price concession}\\
\midrule
year2 $\times$ density&       0.206\sym{***}&       0.040         &       0.064\sym{**} &      -0.019         \\
            &     (0.034)         &     (0.025)         &     (0.028)         &     (0.059)         \\
\addlinespace
year3 $\times$ density&       0.158\sym{***}&       0.089\sym{***}&       0.003         &       0.098\sym{*}  \\
            &     (0.030)         &     (0.023)         &     (0.021)         &     (0.055)         \\
\addlinespace
year4 $\times$ density&       0.059\sym{**} &       0.046\sym{**} &      -0.017         &       0.053         \\
            &     (0.029)         &     (0.022)         &     (0.025)         &     (0.050)         \\
\addlinespace
year5 $\times$ density&       0.089\sym{***}&       0.048\sym{**} &      -0.058\sym{**} &       0.033         \\
            &     (0.031)         &     (0.021)         &     (0.028)         &     (0.046)         \\
\addlinespace
year6 $\times$ density&      -0.184\sym{***}&      -0.008         &      -0.036         &      -0.247\sym{***}\\
            &     (0.054)         &     (0.036)         &     (0.036)         &     (0.087)         \\
\addlinespace
year7 $\times$ density&      -0.133\sym{**} &       0.039         &      -0.035         &      -0.404\sym{***}\\
            &     (0.056)         &     (0.049)         &     (0.041)         &     (0.108)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Lag(Hedonic Control) &  \checkmark         &  \checkmark         &                     &                     \\
\addlinespace
Hedonic Control &                     &                     &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &      134648         &      134648         &     1771638         &     1736077         \\
R-squared   &       0.845         &       0.919         &       0.520         &       0.233         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> result_tables/entry_effect.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(lead times)}&\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{price concession}\\
\midrule
pre2        &      -0.008         &      -0.019\sym{*}  &      -0.015         &      -0.032         \\
            &     (0.014)         &     (0.011)         &     (0.013)         &     (0.026)         \\
\addlinespace
entry       &       0.091\sym{***}&       0.023\sym{***}&      -0.008         &       0.045\sym{**} \\
            &     (0.012)         &     (0.008)         &     (0.009)         &     (0.020)         \\
\addlinespace
post1       &       0.048\sym{***}&       0.031\sym{***}&      -0.012         &       0.045\sym{*}  \\
            &     (0.012)         &     (0.009)         &     (0.010)         &     (0.023)         \\
\addlinespace
post2       &       0.006         &       0.011         &       0.008         &       0.005         \\
            &     (0.013)         &     (0.010)         &     (0.012)         &     (0.024)         \\
\addlinespace
post3       &       0.010         &       0.021\sym{**} &      -0.009         &       0.004         \\
            &     (0.015)         &     (0.011)         &     (0.015)         &     (0.027)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &      103966         &      103966         &      867874         &      845953         \\
R-squared   &       0.815         &       0.912         &       0.506         &       0.227         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> result_tables/entry_effect_hetero_1.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l*{6}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(lead times)}&\multicolumn{1}{c}{log(lead times)}&\multicolumn{1}{c}{log(lead times)}\\
&[lower]&[moderate]&[higher]&[lower]&[moderate]&[higher]\\
\midrule
pre2        &      -0.035         &      -0.031         &       0.004         &      -0.031         &       0.017         &      -0.011         \\
            &     (0.029)         &     (0.033)         &     (0.029)         &     (0.024)         &     (0.028)         &     (0.019)         \\
\addlinespace
entry       &       0.082\sym{***}&       0.067\sym{***}&       0.073\sym{***}&       0.019         &       0.025         &       0.008         \\
            &     (0.029)         &     (0.023)         &     (0.025)         &     (0.022)         &     (0.018)         &     (0.017)         \\
\addlinespace
post1       &       0.056\sym{*}  &       0.015         &       0.023         &       0.036         &       0.018         &       0.039\sym{*}  \\
            &     (0.030)         &     (0.025)         &     (0.026)         &     (0.023)         &     (0.019)         &     (0.021)         \\
\addlinespace
post2       &       0.013         &      -0.005         &       0.022         &       0.054\sym{**} &       0.011         &       0.001         \\
            &     (0.031)         &     (0.025)         &     (0.029)         &     (0.026)         &     (0.022)         &     (0.021)         \\
\addlinespace
post3       &       0.018         &       0.002         &       0.006         &       0.059\sym{**} &      -0.006         &       0.008         \\
            &     (0.034)         &     (0.027)         &     (0.034)         &     (0.024)         &     (0.022)         &     (0.025)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &       31741         &       23336         &       34022         &       31741         &       23336         &       34022         \\
R-squared   &       0.848         &       0.879         &       0.850         &       0.934         &       0.929         &       0.924         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{adjustbox}
}


==> result_tables/entry_effect_hetero_2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l*{6}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{price concession}&\multicolumn{1}{c}{price concession}&\multicolumn{1}{c}{price concession}\\
&[lower]&[moderate]&[higher]&[lower]&[moderate]&[higher]\\
\midrule
pre2        &      -0.028         &      -0.011         &       0.016         &      -0.011         &       0.084         &       0.081         \\
            &     (0.030)         &     (0.034)         &     (0.025)         &     (0.063)         &     (0.077)         &     (0.052)         \\
\addlinespace
entry       &      -0.013         &      -0.045\sym{**} &       0.021         &       0.026         &       0.132\sym{***}&       0.030         \\
            &     (0.022)         &     (0.021)         &     (0.020)         &     (0.060)         &     (0.047)         &     (0.049)         \\
\addlinespace
post1       &      -0.008         &      -0.035\sym{*}  &       0.036         &       0.043         &       0.067         &       0.016         \\
            &     (0.023)         &     (0.020)         &     (0.022)         &     (0.064)         &     (0.056)         &     (0.055)         \\
\addlinespace
post2       &      -0.004         &      -0.029         &       0.057\sym{**} &       0.030         &       0.041         &      -0.017         \\
            &     (0.025)         &     (0.020)         &     (0.025)         &     (0.072)         &     (0.056)         &     (0.061)         \\
\addlinespace
post3       &      -0.021         &      -0.038\sym{*}  &       0.002         &      -0.056         &       0.031         &       0.097         \\
            &     (0.026)         &     (0.022)         &     (0.027)         &     (0.060)         &     (0.056)         &     (0.071)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &      292309         &      242332         &      328835         &      284682         &      236819         &      320074         \\
R-squared   &       0.518         &       0.526         &       0.529         &       0.259         &       0.243         &       0.255         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{adjustbox}
}


==> result_tables/group_1.tex <==
\caption{Panel A: max(closeness centrality)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Beijing   & 0.0174 & 0.0259 & 0.0315 & 0.0338 & 0.035  &        &        \\
 Chengdu   & 0.1365 & 0.2231 & 0.2291 & 0.2675 & 0.282  &        &        \\
 Chongqing & 0.029  & 0.0469 & 0.0483 & 0.0543 & 0.0986 & 0.1006 & 0.0986 \\
 Guangzhou & 0.0317 & 0.0289 & 0.0359 & 0.0357 & 0.0308 & 0.1021 & 0.0932 \\
 Hangzhou  & 0.0556 & 0.0791 & 0.0652 & 0.0584 & 0.085  & 0.0527 & 0.0650 \\
 Nanjing   & 0.0493 & 0.1133 & 0.0868 & 0.1626 & 0.2083 & 0.2073 & 0.1841 \\
 Shanghai  & 0.1132 & 0.0682 & 0.0835 & 0.1024 & 0.0449 & 0.0944 & 0.0376 \\
 Shenzhen  & 0.0362 & 0.0453 & 0.0485 & 0.0379 & 0.0863 &        &        \\
 Tianjin   & 0.0481 & 0.0407 & 0.0371 & 0.0961 & 0.1688 & 0.1837 & 0.1838 \\
 Wuhan     & 0.0259 & 0.0509 & 0.0491 & 0.0357 & 0.0642 &        &        \\
\hline
\end{tabular}

\caption{Panel B: mean(closeness centrality)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Beijing   & 0.0015 & 0.0024 & 0.0025 & 0.0023 & 0.0031 &        &        \\
 Chengdu   & 0.015  & 0.032  & 0.0336 & 0.042  & 0.0415 &        &        \\
 Chongqing & 0.0031 & 0.0036 & 0.0039 & 0.0036 & 0.0073 & 0.0071 & 0.0070 \\
 Guangzhou & 0.0031 & 0.0034 & 0.0029 & 0.0038 & 0.0026 & 0.0079 & 0.0071 \\
 Hangzhou  & 0.0056 & 0.0076 & 0.0055 & 0.0047 & 0.0068 & 0.0039 & 0.0042 \\
 Shenzhen  & 0.003  & 0.0042 & 0.0042 & 0.0039 & 0.0079 &        &        \\
 Shanghai  & 0.0089 & 0.0045 & 0.0064 & 0.0071 & 0.0032 & 0.0060 & 0.0028 \\
 Tianjin   & 0.0053 & 0.0045 & 0.0041 & 0.0071 & 0.0146 & 0.0165 & 0.0164 \\
 Wuhan     & 0.0028 & 0.0039 & 0.003  & 0.0027 & 0.0058 &        &        \\
 Nanjing   & 0.0045 & 0.0113 & 0.008  & 0.0158 & 0.0229 & 0.0202 & 0.0166 \\
\hline
\end{tabular}

\caption{Panel C: median(closeness centrality)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Guangzhou & 0.0003 & 0.0002 & 0.0002 & 0.0002 & 0.0001 & 0.0001 & 0.0001 \\
 Beijing   & 0.0001 & 0      & 0      & 0      & 0      &        &        \\
 Chengdu   & 0.0001 & 0.0001 & 0.0001 & 0      & 0      &        &        \\
 Chongqing & 0.0003 & 0.0002 & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Hangzhou  & 0.0003 & 0.0002 & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Shenzhen  & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 &        &        \\
 Shanghai  & 0      & 0      & 0      & 0      & 0      & 0.0000 & 0.0000 \\
 Tianjin   & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Wuhan     & 0.0004 & 0.0002 & 0.0002 & 0.0001 & 0.0001 &        &        \\
 Nanjing   & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
\hline
\end{tabular}

==> result_tables/group_2.tex <==
\caption{Panel D: max(degree centrality)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Beijing   & 0.0029 & 0.0026 & 0.0027 & 0.0026 & 0.0025 &        &        \\
 Chengdu   & 0.0075 & 0.0064 & 0.0063 & 0.0055 & 0.0061 &        &        \\
 Chongqing & 0.0118 & 0.0121 & 0.0098 & 0.0067 & 0.0052 & 0.0052 & 0.0051 \\
 Guangzhou & 0.0207 & 0.0096 & 0.0121 & 0.0101 & 0.006  & 0.0060 & 0.0061 \\
 Hangzhou  & 0.0126 & 0.0096 & 0.0095 & 0.0079 & 0.0076 & 0.0060 & 0.0065 \\
 Shanghai  & 0.0045 & 0.0034 & 0.0033 & 0.0038 & 0.0038 & 0.0034 & 0.0036 \\
 Shenzhen  & 0.0084 & 0.0076 & 0.0078 & 0.0081 & 0.0075 &        &        \\
 Tianjin   & 0.0092 & 0.0081 & 0.0074 & 0.007  & 0.0079 & 0.0092 & 0.0093 \\
 Wuhan     & 0.0141 & 0.0119 & 0.0105 & 0.0082 & 0.0064 &        &        \\
 Nanjing   & 0.0078 & 0.0071 & 0.0077 & 0.0074 & 0.0069 & 0.0069 & 0.0073 \\
\hline
\end{tabular}

\caption{Panel E: mean(degree centrality)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Shanghai  & 0.0002 & 0.0002 & 0.0002 & 0.0002 & 0.0002 & 0.0002 & 0.0002 \\
 Wuhan     & 0.0009 & 0.0007 & 0.0007 & 0.0005 & 0.0005 &        &        \\
 Tianjin   & 0.0004 & 0.0005 & 0.0004 & 0.0004 & 0.0004 & 0.0005 & 0.0005 \\
 Shenzhen  & 0.0005 & 0.0006 & 0.0005 & 0.0005 & 0.0005 &        &        \\
 Nanjing   & 0.0005 & 0.0006 & 0.0006 & 0.0005 & 0.0005 & 0.0005 & 0.0005 \\
 Hangzhou  & 0.0008 & 0.0006 & 0.0006 & 0.0005 & 0.0005 & 0.0005 & 0.0005 \\
 Guangzhou & 0.0007 & 0.0006 & 0.0007 & 0.0007 & 0.0004 & 0.0005 & 0.0005 \\
 Chongqing & 0.0007 & 0.0007 & 0.0006 & 0.0004 & 0.0004 & 0.0004 & 0.0004 \\
 Chengdu   & 0.0003 & 0.0003 & 0.0003 & 0.0003 & 0.0002 &        &        \\
 Beijing   & 0.0002 & 0.0002 & 0.0002 & 0.0002 & 0.0002 &        &        \\
\hline
\end{tabular}

\caption{Panel F: median(degree centrality)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Beijing   & 0.0001 & 0      & 0      & 0      & 0      &        &        \\
 Chengdu   & 0.0001 & 0.0001 & 0.0001 & 0      & 0      &        &        \\
 Chongqing & 0.0003 & 0.0002 & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Guangzhou & 0.0003 & 0.0002 & 0.0002 & 0.0002 & 0.0001 & 0.0001 & 0.0001 \\
 Hangzhou  & 0.0003 & 0.0002 & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Nanjing   & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Shanghai  & 0      & 0      & 0      & 0      & 0      & 0.0000 & 0.0000 \\
 Shenzhen  & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 &        &        \\
 Tianjin   & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Wuhan     & 0.0004 & 0.0002 & 0.0002 & 0.0001 & 0.0001 &        &        \\
\hline
\end{tabular}

==> result_tables/group_3.tex <==
\caption{Panel G: max(page rank)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Beijing   & 0.0014 & 0.0011 & 0.0011 & 0.001  & 0.0007 &        &        \\
 Chengdu   & 0.0036 & 0.0025 & 0.0021 & 0.0018 & 0.0011 &        &        \\
 Guangzhou & 0.0102 & 0.0041 & 0.0042 & 0.0059 & 0.0024 & 0.0012 & 0.0011 \\
 Hangzhou  & 0.0067 & 0.0042 & 0.0034 & 0.0042 & 0.0016 & 0.0015 & 0.0016 \\
 Chongqing & 0.0085 & 0.0069 & 0.0045 & 0.0034 & 0.0019 & 0.0014 & 0.0011 \\
 Shanghai  & 0.0011 & 0.0013 & 0.001  & 0.0008 & 0.001  & 0.0018 & 0.0013 \\
 Shenzhen  & 0.0046 & 0.0023 & 0.0024 & 0.0037 & 0.0012 &        &        \\
 Tianjin   & 0.0048 & 0.0038 & 0.0052 & 0.0043 & 0.0021 & 0.0017 & 0.0016 \\
 Wuhan     & 0.0085 & 0.0044 & 0.0032 & 0.0031 & 0.0011 &        &        \\
 Nanjing   & 0.005  & 0.0022 & 0.0024 & 0.0023 & 0.0016 & 0.0014 & 0.0011 \\
\hline
\end{tabular}

\caption{Panel H: mean(page rank)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Beijing   & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 &        &        \\
 Chengdu   & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 &        &        \\
 Guangzhou & 0.0007 & 0.0003 & 0.0004 & 0.0004 & 0.0002 & 0.0001 & 0.0001 \\
 Hangzhou  & 0.0005 & 0.0004 & 0.0004 & 0.0003 & 0.0002 & 0.0002 & 0.0002 \\
 Chongqing & 0.0006 & 0.0005 & 0.0004 & 0.0003 & 0.0002 & 0.0001 & 0.0001 \\
 Shanghai  & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Shenzhen  & 0.0003 & 0.0003 & 0.0003 & 0.0003 & 0.0002 &        &        \\
 Tianjin   & 0.0003 & 0.0003 & 0.0003 & 0.0002 & 0.0001 & 0.0001 & 0.0001 \\
 Wuhan     & 0.0007 & 0.0004 & 0.0003 & 0.0002 & 0.0001 &        &        \\
 Nanjing   & 0.0003 & 0.0003 & 0.0003 & 0.0002 & 0.0002 & 0.0001 & 0.0001 \\
\hline
\end{tabular}

\caption{Panel I: median(page rank)}
\begin{tabular}{lrrrrrll}
\hline
 city      &   2016 &   2017 &   2018 &   2019 &   2020 & 2021   & 2022   \\
\hline
 Tianjin   & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0      & 0.0000 & 0.0000 \\
 Beijing   & 0      & 0      & 0      & 0      & 0      &        &        \\
 Chengdu   & 0.0001 & 0      & 0      & 0      & 0      &        &        \\
 Chongqing & 0.0003 & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0000 & 0.0000 \\
 Guangzhou & 0.0003 & 0.0001 & 0.0001 & 0.0002 & 0.0001 & 0.0000 & 0.0000 \\
 Hangzhou  & 0.0002 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
 Nanjing   & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0000 & 0.0000 \\
 Shanghai  & 0      & 0      & 0      & 0      & 0      & 0.0000 & 0.0000 \\
 Shenzhen  & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 &        &        \\
 Wuhan     & 0.0003 & 0.0001 & 0.0001 & 0.0001 & 0      &        &        \\
\hline
\end{tabular}

==> result_tables/heter_platform_did_1.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l*{6}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(lead times)}&\multicolumn{1}{c}{log(lead times)}&\multicolumn{1}{c}{log(lead times)}\\
&[lower]&[moderate]&[higher]&[lower]&[moderate]&[higher]\\
\midrule
pre1\_treatment&      -0.016         &      -0.012         &       0.016         &       0.017         &       0.015         &      -0.033         \\
            &     (0.021)         &     (0.015)         &     (0.029)         &     (0.015)         &     (0.013)         &     (0.024)         \\
\addlinespace
treatment   &      -0.029\sym{*}  &      -0.002         &       0.019         &       0.006         &      -0.002         &      -0.011         \\
            &     (0.017)         &     (0.016)         &     (0.032)         &     (0.016)         &     (0.013)         &     (0.024)         \\
\addlinespace
post1\_treatment&       0.041\sym{*}  &       0.071\sym{***}&       0.049         &       0.046\sym{**} &       0.035\sym{**} &      -0.007         \\
            &     (0.022)         &     (0.018)         &     (0.035)         &     (0.018)         &     (0.014)         &     (0.025)         \\
\addlinespace
post2\_treatment&       0.062\sym{***}&       0.077\sym{***}&       0.028         &       0.040\sym{*}  &       0.028\sym{*}  &      -0.015         \\
            &     (0.022)         &     (0.021)         &     (0.041)         &     (0.021)         &     (0.016)         &     (0.029)         \\
\addlinespace
post3\_treatment&      -0.002         &       0.067\sym{***}&       0.039         &       0.027         &      -0.006         &      -0.025         \\
            &     (0.025)         &     (0.025)         &     (0.069)         &     (0.023)         &     (0.019)         &     (0.046)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &       41849         &       53806         &       24273         &       41849         &       53806         &       24273         \\
R-squared   &       0.850         &       0.871         &       0.894         &       0.935         &       0.927         &       0.938         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{adjustbox}
}


==> result_tables/heter_platform_did_2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l*{6}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{price concession}&\multicolumn{1}{c}{price concession}&\multicolumn{1}{c}{price concession}\\
&[lower]&[moderate]&[higher]&[lower]&[moderate]&[higher]\\
\midrule
pre1\_treatment&       0.001         &      -0.002         &      -0.044\sym{*}  &       0.012         &      -0.011         &      -0.017         \\
            &     (0.017)         &     (0.016)         &     (0.025)         &     (0.041)         &     (0.034)         &     (0.049)         \\
\addlinespace
treatment   &       0.001         &      -0.004         &       0.014         &       0.017         &      -0.017         &      -0.019         \\
            &     (0.021)         &     (0.016)         &     (0.030)         &     (0.041)         &     (0.036)         &     (0.060)         \\
\addlinespace
post1\_treatment&       0.001         &      -0.015         &       0.005         &       0.084\sym{*}  &       0.026         &       0.020         \\
            &     (0.025)         &     (0.020)         &     (0.031)         &     (0.050)         &     (0.041)         &     (0.066)         \\
\addlinespace
post2\_treatment&      -0.002         &      -0.022         &      -0.013         &       0.160\sym{***}&       0.068         &       0.092         \\
            &     (0.027)         &     (0.023)         &     (0.029)         &     (0.056)         &     (0.048)         &     (0.077)         \\
\addlinespace
post3\_treatment&      -0.004         &      -0.011         &       0.026         &       0.034         &       0.118\sym{*}  &      -0.086         \\
            &     (0.031)         &     (0.026)         &     (0.040)         &     (0.067)         &     (0.067)         &     (0.130)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &      333284         &      587056         &      345003         &      328031         &      576728         &      338698         \\
R-squared   &       0.548         &       0.538         &       0.529         &       0.255         &       0.247         &       0.270         \\
\bottomrule
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
\end{adjustbox}
}


==> result_tables/mccrary_results.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Tue Jul  9 09:10:37 2024
\begin{table}[ht]
  \centering
  \caption{McCrary Test Results} 
  \label{tab:mccrary_results}
  \begin{tabular}{rrrrrr}
    \hline
   & Bandwidth & Log\_Diff & SE & Z\_Stat & P\_Value \\ 
    \hline
  1 & 0.05 & -0.03 & 0.03 & -0.94 & 0.35 \\ 
    2 & 0.06 & -0.03 & 0.03 & -1.08 & 0.28 \\ 
    3 & 0.03 & 0.04 & 0.04 & 1.17 & 0.24 \\ 
    4 & 0.03 & 0.00 & 0.04 & 0.07 & 0.95 \\ 
    5 & 0.08 & -0.02 & 0.02 & -0.75 & 0.45 \\ 
    6 & 0.07 & -0.03 & 0.03 & -1.07 & 0.28 \\ 
    7 & 0.04 & -0.02 & 0.03 & -0.54 & 0.59 \\ 
    8 & 0.04 & -0.01 & 0.03 & -0.16 & 0.87 \\ 
     \hline
  \end{tabular}

  \end{table}

==> result_tables/movement_cutoff.tex <==
% latex table generated in R 4.2.0 by xtable 1.8-4 package
% Mon Jul  8 21:20:28 2024
\begin{table}[ht]
\centering
\caption{Placebo Test Results for Different Cutoff Point} 
\label{tab:movement_cutoff}
\begin{tabular}{rlllllr}
  \hline
Cutoff & Estimate & SE & Z & PValue & Bandwidth & EffectiveObs \\ 
  \hline
0.32 & -33154 & 16261 & -2.04 & 0.0415 & 0.0965 & 58710 \\ 
  0.35 & 2112 & 13951 & 0.151 & 0.88 & 0.132 & 75514 \\ 
  0.40 & -25930 & 19778 & -1.31 & 0.19 & 0.0764 & 38332 \\ 
  0.42 & -12532 & 18043 & -0.695 & 0.487 & 0.0855 & 40529 \\ 
  0.45 & -22806 & 17952 & -1.27 & 0.204 & 0.0858 & 36968 \\ 
  0.50 & 25778 & 15534 & 1.66 & 0.097 & 0.133 & 49373 \\ 
  0.65 & 47140 & 21425 & 2.2 & 0.0278 & 0.092 & 20096 \\ 
  0.70 & -32584 & 19286 & -1.69 & 0.0911 & 0.121 & 22549 \\ 
   \hline
\end{tabular}
\end{table}



==> result_tables/quantile_network_formation_1.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{10}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
            &\multicolumn{1}{c}{FE}&\multicolumn{1}{c}{Q(5)}&\multicolumn{1}{c}{Q(10)}&\multicolumn{1}{c}{Q(15)}&\multicolumn{1}{c}{Q(20)}&\multicolumn{1}{c}{Q(25)}&\multicolumn{1}{c}{Q(30)}&\multicolumn{1}{c}{Q(35)}&\multicolumn{1}{c}{Q(40)}&\multicolumn{1}{c}{Q(45)}\\
\midrule
pre1\_treatment&      -0.063\sym{*}  &       0.034         &       0.017         &       0.005         &      -0.003         &      -0.009         &      -0.017         &      -0.026         &      -0.037         &      -0.049         \\
            &     (0.033)         &     (0.584)         &     (0.518)         &     (0.473)         &     (0.441)         &     (0.416)         &     (0.388)         &     (0.352)         &     (0.312)         &     (0.267)         \\
\addlinespace
treatment   &       0.777\sym{***}&       0.878         &       0.860\sym{*}  &       0.848\sym{*}  &       0.840\sym{**} &       0.833\sym{**} &       0.826\sym{**} &       0.816\sym{**} &       0.805\sym{***}&       0.793\sym{***}\\
            &     (0.049)         &     (0.553)         &     (0.491)         &     (0.448)         &     (0.417)         &     (0.394)         &     (0.368)         &     (0.333)         &     (0.295)         &     (0.252)         \\
\addlinespace
post1\_treatment&       1.230\sym{***}&       1.433\sym{**} &       1.398\sym{**} &       1.373\sym{***}&       1.356\sym{***}&       1.343\sym{***}&       1.328\sym{***}&       1.308\sym{***}&       1.286\sym{***}&       1.261\sym{***}\\
            &     (0.068)         &     (0.650)         &     (0.577)         &     (0.527)         &     (0.491)         &     (0.463)         &     (0.432)         &     (0.392)         &     (0.347)         &     (0.297)         \\
\addlinespace
post2\_treatment&       1.618\sym{***}&       1.626\sym{**} &       1.625\sym{**} &       1.624\sym{**} &       1.623\sym{***}&       1.622\sym{***}&       1.622\sym{***}&       1.621\sym{***}&       1.620\sym{***}&       1.619\sym{***}\\
            &     (0.088)         &     (0.802)         &     (0.712)         &     (0.650)         &     (0.605)         &     (0.572)         &     (0.533)         &     (0.483)         &     (0.428)         &     (0.366)         \\
\addlinespace
post3\_treatment&       1.731\sym{***}&       1.689         &       1.697         &       1.702         &       1.705\sym{*}  &       1.708\sym{*}  &       1.711\sym{**} &       1.715\sym{**} &       1.720\sym{**} &       1.725\sym{***}\\
            &     (0.123)         &     (1.281)         &     (1.137)         &     (1.039)         &     (0.967)         &     (0.913)         &     (0.852)         &     (0.772)         &     (0.684)         &     (0.585)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &      133818         &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         \\
\bottomrule
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> result_tables/quantile_network_formation_2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{10}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
            &\multicolumn{1}{c}{Q(50)}&\multicolumn{1}{c}{Q(55)}&\multicolumn{1}{c}{Q(60)}&\multicolumn{1}{c}{Q(65)}&\multicolumn{1}{c}{Q(70)}&\multicolumn{1}{c}{Q(75)}&\multicolumn{1}{c}{Q(80)}&\multicolumn{1}{c}{Q(85)}&\multicolumn{1}{c}{Q(90)}&\multicolumn{1}{c}{Q(95)}\\
\midrule
pre1\_treatment&      -0.062         &      -0.076         &      -0.089         &      -0.101         &      -0.111         &      -0.119         &      -0.127         &      -0.139         &      -0.153         &      -0.173         \\
            &     (0.216)         &     (0.166)         &     (0.124)         &     (0.092)         &     (0.078)         &     (0.080)         &     (0.095)         &     (0.128)         &     (0.173)         &     (0.247)         \\
\addlinespace
treatment   &       0.779\sym{***}&       0.764\sym{***}&       0.751\sym{***}&       0.739\sym{***}&       0.728\sym{***}&       0.720\sym{***}&       0.711\sym{***}&       0.699\sym{***}&       0.685\sym{***}&       0.664\sym{***}\\
            &     (0.205)         &     (0.157)         &     (0.117)         &     (0.087)         &     (0.073)         &     (0.076)         &     (0.090)         &     (0.121)         &     (0.164)         &     (0.233)         \\
\addlinespace
post1\_treatment&       1.233\sym{***}&       1.204\sym{***}&       1.177\sym{***}&       1.152\sym{***}&       1.129\sym{***}&       1.114\sym{***}&       1.096\sym{***}&       1.071\sym{***}&       1.044\sym{***}&       1.001\sym{***}\\
            &     (0.240)         &     (0.185)         &     (0.138)         &     (0.102)         &     (0.086)         &     (0.090)         &     (0.106)         &     (0.142)         &     (0.192)         &     (0.274)         \\
\addlinespace
post2\_treatment&       1.618\sym{***}&       1.617\sym{***}&       1.616\sym{***}&       1.615\sym{***}&       1.614\sym{***}&       1.613\sym{***}&       1.613\sym{***}&       1.612\sym{***}&       1.610\sym{***}&       1.609\sym{***}\\
            &     (0.297)         &     (0.228)         &     (0.170)         &     (0.126)         &     (0.106)         &     (0.110)         &     (0.130)         &     (0.175)         &     (0.237)         &     (0.338)         \\
\addlinespace
post3\_treatment&       1.731\sym{***}&       1.737\sym{***}&       1.742\sym{***}&       1.747\sym{***}&       1.752\sym{***}&       1.755\sym{***}&       1.759\sym{***}&       1.764\sym{***}&       1.770\sym{***}&       1.779\sym{***}\\
            &     (0.474)         &     (0.365)         &     (0.271)         &     (0.202)         &     (0.170)         &     (0.176)         &     (0.208)         &     (0.280)         &     (0.379)         &     (0.541)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         &      142734         \\
\bottomrule
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> result_tables/rdd_placebo_test.tex <==
% latex table generated in R 4.2.0 by xtable 1.8-4 package
% Mon Jul  8 21:18:14 2024
\begin{table}[ht]
\centering
\caption{Placebo Test Results for Different Covariates} 
\label{tab:placebo_test_results}
\begin{tabular}{llllllr}
  \hline
Covariate & Estimate & SE & Z & PValue & Bandwidth & EffectiveObs \\ 
  \hline
pop & -61.8 & 405 & -0.153 & 0.879 & 0.063 & 30518 \\ 
  light & -0.229 & 0.266 & -0.859 & 0.39 & 0.063 & 30518 \\ 
  price\_concession & -0.000412 & 0.000756 & -0.546 & 0.585 & 0.063 & 29974 \\ 
  ln\_end\_price & -0.0248 & 0.0171 & -1.45 & 0.147 & 0.063 & 30518 \\ 
  ln\_nego\_changes & 0.000749 & 0.0227 & 0.033 & 0.974 & 0.063 & 30518 \\ 
  ln\_watch\_time & 0.0673 & 0.0699 & 0.962 & 0.336 & 0.063 & 30518 \\ 
  green\_ratio & -0.00135 & 0.00236 & -0.572 & 0.568 & 0.063 & 30518 \\ 
  bedroom & -0.00953 & 0.0181 & -0.528 & 0.598 & 0.063 & 30518 \\ 
  ln\_watch\_people & 0.0527 & 0.0366 & 1.44 & 0.15 & 0.063 & 30518 \\ 
  living\_room & 0.000967 & 0.0116 & 0.0834 & 0.934 & 0.063 & 30518 \\ 
  ln\_negotiation\_period & -0.00619 & 0.0273 & -0.227 & 0.821 & 0.063 & 30518 \\ 
  museum & -0.0603 & 0.0425 & -1.42 & 0.156 & 0.063 & 30518 \\ 
  kind & -0.0047 & 0.139 & -0.0338 & 0.973 & 0.063 & 30518 \\ 
  mid & 0.0126 & 0.0623 & 0.203 & 0.839 & 0.063 & 30518 \\ 
  total\_building & -0.269 & 0.847 & -0.318 & 0.751 & 0.063 & 30518 \\ 
  total\_resident & 8.27 & 21 & 0.395 & 0.693 & 0.063 & 30518 \\ 
  green\_ratio & -0.00135 & 0.00236 & -0.572 & 0.568 & 0.063 & 30518 \\ 
  old & 0.0444 & 0.0433 & 1.02 & 0.305 & 0.063 & 30518 \\ 
  house\_age & 0.147 & 0.282 & 0.523 & 0.601 & 0.063 & 30518 \\ 
  total\_building & -0.269 & 0.847 & -0.318 & 0.751 & 0.063 & 30518 \\ 
   \hline
\end{tabular}
\end{table}



==> result_tables/rdd_result_summary.tex <==
% latex table generated in R 4.2.0 by xtable 1.8-4 package
% Mon Jul  8 21:12:27 2024
\begin{table}[ht]
\centering

\caption{RD Estimates with Different Bandwidth Selection Methods and Kernels} 
\label{tab:rd_bandwidth_kernel_results}
\begin{tabular}{lllllllr}
  \hline
Method & Kernel & Estimate & SE & Z & PValue & Bandwidth & EffectiveObs \\ 
  \hline
mserd & uniform & -48903 & 21529 & -2.27 & 0.0231 & 0.0504 & 24269 \\ 
  mserd & triangular & -61304 & 20887 & -2.94 & 0.00333 & 0.063 & 30532 \\ 
  cerrd & uniform & -56899 & 28636 & -1.99 & 0.0469 & 0.0273 & 13166 \\ 
  cerrd & triangular & -59561 & 27943 & -2.13 & 0.033 & 0.0341 & 16392 \\ 
   \hline
\end{tabular}
\end{table}



==> result_tables/rdd_result_summary_robust.tex <==
% latex table generated in R 4.2.0 by xtable 1.8-4 package
% Mon Jul  8 21:13:07 2024
\begin{table}[ht]
\centering
\caption{RD Estimates with Different Bandwidth Selection Methods and Kernels (robust method with log(income))} 
\label{tab:rd_bandwidth_kernel_results_robust}
\begin{tabular}{lllllllr}
  \hline
Method & Kernel & Estimate & SE & Z & PValue & Bandwidth & EffectiveObs \\ 
  \hline
mserd & uniform & -0.0584 & 0.0263 & -2.22 & 0.0263 & 0.0773 & 37645 \\ 
  mserd & triangular & -0.0697 & 0.0314 & -2.22 & 0.0267 & 0.066 & 32020 \\ 
  cerrd & uniform & -0.0874 & 0.0361 & -2.42 & 0.0156 & 0.0418 & 19988 \\ 
  cerrd & triangular & -0.0663 & 0.0434 & -1.53 & 0.126 & 0.0357 & 17191 \\ 
   \hline
\end{tabular}
\end{table}



==> result_tables/robustness_more_entry_resuls.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{log(visits)}&\multicolumn{1}{c}{log(visits)}&\multicolumn{1}{c}{log(transaction time)}&\multicolumn{1}{c}{log(transaction time)}\\
\midrule
entry\_flag  &       0.015\sym{**} &                     &      -0.007         &                     \\
            &     (0.006)         &                     &     (0.008)         &                     \\
\addlinespace
pre2        &                     &      -0.027\sym{***}&                     &      -0.014         \\
            &                     &     (0.008)         &                     &     (0.013)         \\
\addlinespace
entry       &                     &       0.019\sym{***}&                     &      -0.011         \\
            &                     &     (0.007)         &                     &     (0.009)         \\
\addlinespace
post1       &                     &       0.010         &                     &      -0.016         \\
            &                     &     (0.007)         &                     &     (0.010)         \\
\addlinespace
post2       &                     &       0.001         &                     &       0.004         \\
            &                     &     (0.009)         &                     &     (0.012)         \\
\addlinespace
post3       &                     &      -0.009         &                     &      -0.012         \\
            &                     &     (0.008)         &                     &     (0.015)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &      867874         &      867874         &      867874         &      867874         \\
R-squared   &       0.777         &       0.777         &       0.506         &       0.506         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> result_tables/robustness_more_plat_resuls.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{log(visits)}&\multicolumn{1}{c}{log(visits)}&\multicolumn{1}{c}{log(transaction time)}&\multicolumn{1}{c}{log(transaction time)}\\
\midrule
treatment\_flag&       0.005         &                     &       0.000         &                     \\
            &     (0.005)         &                     &     (0.010)         &                     \\
\addlinespace
pre2\_treatment&                     &      -0.001         &                     &       0.011         \\
            &                     &     (0.005)         &                     &     (0.008)         \\
\addlinespace
treatment   &                     &      -0.002         &                     &       0.005         \\
            &                     &     (0.005)         &                     &     (0.009)         \\
\addlinespace
post1\_treatment&                     &       0.017\sym{***}&                     &       0.009         \\
            &                     &     (0.006)         &                     &     (0.012)         \\
\addlinespace
post2\_treatment&                     &       0.016\sym{**} &                     &       0.007         \\
            &                     &     (0.007)         &                     &     (0.015)         \\
\addlinespace
post3\_treatment&                     &       0.009         &                     &       0.005         \\
            &                     &     (0.010)         &                     &     (0.017)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Hedonic Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &     1268778         &     1268778         &     1268778         &     1268778         \\
R-squared   &       0.776         &       0.776         &       0.528         &       0.528         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> result_tables/stylized_fact.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{log(number)}&\multicolumn{1}{c}{log(lead times)}&\multicolumn{1}{c}{log(negotiation period)}&\multicolumn{1}{c}{price concession}\\
\midrule
density     &       0.070\sym{***}&       0.042\sym{***}&       0.011         &       0.028         \\
            &     (0.020)         &     (0.015)         &     (0.015)         &     (0.033)         \\
\addlinespace
Brokerage Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Lag(Hedonic Control) &  \checkmark         &  \checkmark         &                     &                     \\
\addlinespace
Hedonic Control &                     &                     &  \checkmark         &  \checkmark         \\
\addlinespace
Transaction Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\addlinespace
Regional Control &  \checkmark         &  \checkmark         &  \checkmark         &  \checkmark         \\
\midrule
\(N\)       &      134648         &      134648         &     1771638         &     1736077         \\
R-squared   &       0.844         &       0.918         &       0.520         &       0.233         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> sections/mechanism.tex <==
In the context of the real estate market, it is evident that real estate is not a homogeneous good. Consequently, the brokerage market is distinguished by the presence of a considerable number of firms, exhibiting minimal barriers to entry. The prevailing economic theory posits that such a market, typified by robust competition, a multitude of firms, and a relatively low market concentration, is consistent with empirical observations. For instance, Lianjia's physical locations account for less than 5\% of the total, yet Lianjia handles approximately 20\% of the national transactions. Furthermore, numerous prominent agencies, such as Woaiwojia and Centaline Property Agency, operate within this market, indicating a monopolistic competitive environment.

Nevertheless, when examining local segmented markets, the monopolistic competition model appears to be less pertinent. In local markets, the surrounding neighborhoods exhibit a high degree of homogeneity with respect to community characteristics and the availability of public resources. In particular, apartments are the most favored property type in the Chinese real estate market, characterized by minimal inherent differences, making them relatively homogeneous goods. Furthermore, local real estate markets exhibit no barriers to entry or exit, closely resembling perfect competition. From a cost perspective, the real estate market has undergone platform-mediated reforms, whereby data resources exhibit zero marginal cost characteristics and operating costs decrease in line with the expansion of the user base. This suggests the presence of characteristics associated with a natural monopoly. In light of these circumstances, the operational stance of firms diverges considerably from that observed in a monopolistically competitive market. The presence of network effects gives rise to a virtuous cycle wherein an expansion in the number of branches of a dominant real estate agency draws in a greater number of users, which in turn attracts a greater volume of real estate listings. This positive feedback loop serves to reinforce the dominant position of firms like Lianjia, ultimately leading to the formation of oligopolistic firms. These oligopolistic firms are then able to sustain and reinforce their dominant market positions.

In local segmented markets, oligopolistic firms are responsible for increasing network strength and possess considerable market power. In segmented markets where some oligopolistic firms do not have strong network effects, multiple other firms serve the diverse needs of consumers and expand their scale. The real estate brokerage market is characterised by an inclusive competitive landscape, which can be attributed to a number of factors, including free entry, rapid technological progress and business model innovation. This environment allows oligopolistic firms to either enhance the strength of their network effects or face challenges to their dominant positions. Consequently, monopolistic structures emerge from and are subsequently disrupted by competition, thereby enabling real estate intermediaries to continuously evolve and drive the industry's rapid growth. In practical terms, this suggests that a competitive oligopolistic structure does not inherently impede competitive efficiency. Rather, as our empirical findings indicate, the enriched entry and transformations within the market lead to an increase in the number of transactions and house tours. This type of market structure can enhance firm efficiency, thereby facilitating more efficient transactions for buyers and sellers and improving overall market welfare, even though it may impede individual seller welfare. Moreover, this form of competition predominantly occurs among different brands within the larger platform, while the broader monopolistic or oligopolistic structure remains largely insulated from the competitive pressures posed by new entrants.

As evidenced by our empirical findings, Lianjia's strategic approach has markedly augmented its network strength within the context of segmented markets. From this perspective, the enhancement of network effects further drives the segmented market toward an oligopolistic competitive structure, which could increase market welfare and facilitate transactions between buyers and sellers. Furthermore, with the advent of online platforms and novel technologies, such as Lianjia's cutting-edge virtual reality (VR) home viewing technology, these network effects are gradually shifting from local networks to a global network. Consequently, this development is transforming the overall market into an oligopolistic competition model on a larger scale.

As network effects intensify in the future, the real estate brokerage market may witness a more pronounced consolidation of market power among a few dominant players. This consolidation may result in increased efficiencies through economies of scale and scope, whereby firms utilize their extensive data resources and technological advancements to optimize operations and enhance consumer experiences. Nevertheless, this transition gives rise to significant considerations for regulatory authorities, with a view to guaranteeing that the market remains competitive and accessible. The dynamic interplay between technological innovation and market structure will be of more crucial. As firms such as Lianjia persist in their efforts to innovate, incorporating artificial intelligence, big data analytics, and blockchain technology for secure transactions, the real estate market may become more transparent and efficient. Such developments could reduce transaction costs, diminish information asymmetry, and furnish consumers with more personalized services. Moreover, the global reach of network effects suggests that real estate brokerage markets across disparate regions may become more interconnected. This interconnectivity could facilitate cross-city or cross-province investments and diversify property portfolios for investors, thereby contributing to a more resilient real estate market.

In conclusion, the evolution of the real estate brokerage market towards an oligopolistic competition model, driven by network effects and technological advancements, presents both opportunities and challenges. Our empirical findings indicate that this type of market structure does not impede competitive efficiencies. However, policymakers and industry stakeholders must navigate this landscape carefully to harness the benefits of increased efficiency and innovation while safeguarding against potential market power abuses and ensuring equitable access for all participants. A balanced approach to these issues will be essential for sustaining long-term growth and enhancing overall market welfare in the real estate industry.


==> sections/stylized_fact_unused_.tex <==

\subsection{Stylized Fact} \label{subsec:stylized_fact}

% To quantify Lianjia's impact, we begin by establishing a key stylized fact, which we develop a Density-Based Index (DBI) index to capture the Lianjia's offline stores' influential ratio. The index is to measure the effects of Lianjia's operations and its continuous expansion. The definition of this index is informed by the results of an influential radius test, which helps us capture the spatial extent of Lianjia's influence on local real estate markets. This approach allows for a more nuanced understanding of how Lianjia's presence affects key market variables. The DBI is calculated as follows:

We also develop a Density-Based Index (DBI) index to capture the Lianjia's offline stores' influential ratio. The index is to measure the effects of Lianjia's operations and its continuous expansion. The definition of this index is informed by the results of an influential radius test, which helps us capture the spatial extent of Lianjia's influence on local real estate markets. This approach allows for a more nuanced understanding of how Lianjia's presence affects key market variables. The DBI is calculated as follows:


\begin{equation*}
  density_{it} = \frac{lianjia_{it}}{total_{it}},
\end{equation*}

where $lianjia_{it}$ represents the number of Lianjia's stores within a 410-meter radius and $total_{it}$ denotes the total number of real estate brokerages' stores within the same radius. The choice of this index is grounded in an effort to address potential reverse causality issues. Specifically, Lianjia and other brokerages often strategically place their stores in highly desirable locations, which typically also results high transaction volumes. This could potentially will caused our estimation biased if we were to simply count the number of Lianjia's stores. To deal for this issue, we employ a comparative metric: the ratio of Lianjia brokerages to the total number of real estate brokerages within the radius. This ratio helps mitigate the bias that may arise from the strategic location choices of Lianjia, offering a clearer measure of its market influence relative to competitors. This approach aligns with the principles of spatial competition theory, as articulated by \citep{hotelling_stability_1929, daspremont_hotellings_1979} in competition model. Such a comparative metric not only provides a more accurate reflection of Lianjia's market penetration but also adheres to economic modeling standards by accounting for competitive dynamics in the sector.

To capture the individual fixed effect and other time-invariant unobservable influential factors, a multi-way fixed effect model is proposed. The model is specified as follows: 

\begin{equation}
  Y_{it} = \beta_0 + \beta_1 density_{it} + \bf{\alpha} \bf{X}_{it} + \eta_{t} \times \text{bs\_code}_i + \mu_i + \epsilon_{it}, \label{eq:multi-way-fe}
\end{equation}

where $Y_{it}$ is the three main dependent variables, including $\log(\text{number})$, price concession, and $\log(\text{lead times})$, $density_{it}$ is the DBI, $\bf{X}_{it}$ are a set of control variables, including brokerage\_control Lag(hedonic\_control), transaction\_control and region\_control, while $\eta_{t} \times \text{bs\_code}_i$ is the time dummy variable interacting with the fixed effect of the business area, $\mu_i$ is the neighborhood fixed effect and $\epsilon_{it}$ is the random error term. The standard errors are clustered at the each business area level.\footnote{The business area is defined as a zone with combination of multiple neighborhoods, which Lianjia designates as the primary divisions of the entire region. The Lianjia's definition of a zone is different and typically smaller than a zone defined by the government.} The results are shown in Table \ref{tab:stylized_fact}.

\begin{table}[htb!]
    \centering
    \begin{scriptsize}
    \input{result_tables/stylized_fact}
    \caption{The DBI Influence to the Lianjia's Transaction}

    Note: we omit all the control variables in the regression model, and detailed descriptions can be seen from Table \ref{tab:statistical_district} and Table \ref{tab:statistical_individual}. In column 1 and 2, we estimated the model using the neighborhood-level data and in column 3 and 4, we estimated the model using the individual-level data, respectively. Standard Errors are clustered at the business area level.
    \label{tab:stylized_fact}
    \end{scriptsize}
\end{table}

The results show that the share of Linajia's offline stores in total brokerage plays a significant role in the real estate market, especially in terms of number and lead time, but not in terms of price concession and transaction period. Specifically, a 1\% increase in a Lianjia's DBI within an area correlates with a 7\% increase in number, as indicated in column 1. Furthermore, this increased DBI also leads to a 4.2\% increase in the number of home tours in the column 2, underscoring the Lianjia's increased visibility and potential for customer engagement. In contrast, the analysis shows no significant effect of DBI on price concessions and transaction time. This finding suggests that while a larger share of offline stores within the segmented market increases the number of sales and the number of house tours, it may not be beneficial for mathcing the buyers and sellers, as demonstrated by the insignificance of the coefficients of log(transaction period) and price concessions. The broader implications point to the strategic advantage of density or market share in driving business performance metrics, except for customers' choices, which appear to be unaffected by changes in market share.

Within the temporal scope of our investigation, the dataset encapsulates two distinct epochs: a phase characterized by surging housing prices and the subsequent period marked by the COVID-19 pandemic. These intervals were further complicated by regulatory measures enacted by the Chinese government, significantly altering the operational dynamics and influence of brokerages within the housing market. Acknowledging these temporal shifts necessitates a nuanced analysis of the brokerage effect across different stages of the study period to ensure the robustness of our findings. To address this, we adopt a dynamic analytical approach, dissecting the period into annual segments. This granularity is achieved by constructing seven unique variables, each representing the interaction between brokerage density and the respective $density_{it} * year_{it}$. Our methodology employs a multi-way fixed effects model, as detailed in Equation \eqref{eq:dynamic}, which facilitates a comprehensive examination of temporal variations in the brokerage's market impact.

In the construction of our regression model, we deliberately omit the first period to avoid multicollinearity problem, treating it as a baseline for comparison. This strategic choice allows us to refine our proxy variable—the product of Lianjia's Dealership Balance Index (DBI) and annual dummies—as a better measure of Lianjia's local market power. Besides, to control potential self correlation problem, we also included lagged one period dependent variables in the model. Other settings are the same with the previous model \eqref{eq:multi-way-fe} and the model is described as \eqref{eq:dynamic} and the results are reported in Table \ref{tab:Dynamic}: 

\begin{equation}
  Y_{it} = \beta_0 + \rho Y_{it-1} + \sum_{i=2}^7 density_{it} * year_{it} + \bf{\alpha} \bf{X}_{it} + \eta_{t} \times \text{bs\_code}_i + \mu_i + \epsilon_{it}. \label{eq:dynamic}
\end{equation}

\begin{table}[H]
  \begin{center}
    \begin{scriptsize}
    \caption{Dynamic Regression Results}
    \label{tab:Dynamic}
    \input{result_tables/dynamic.tex}

    Note: we omit all the control variables in the regression model, and detailed descriptions can be seen from Table \ref{tab:statistical_district} and Table \ref{tab:statistical_individual}. Standard Errors are clustered at the business area level.
    \end{scriptsize}
  \end{center}
\end{table}

The result highlights the dynamic impact of offline store's share on market performance, especially in response to external factors such as the digital transformation and the COVID-19 pandemic. Firstly, Lianjia's impact on transaction number showed a significant decreasing trend, but remains significantly positive before the 2020. However, the impact of offline stores turned significantly negative in 2020 and 2021, coinciding with the outbreak of the COVID-19 pandemic. The widespread restrictions during this period severely disrupted Lianjia's offline transaction procedures and business activities, highlighting the vulnerability of real estate transactions to macroeconomic shocks. In terms of number of home tours, Lianjia's impact remained positive from 2018 to 2020. This period coincides with Lianjia's online platform consolidation period where Lianjia decides to adopt the online platform consolidation strategy, where the offline stores have more incentives to attract more buyers to visit their stores. This suggests that a strong market presence correlates with increased buyer attention, which translates into more home tours. However, pandemic-related restrictions dampened this effect in later years, highlighting the challenges posed by external constraints on physical real estate activity. Regarding the transaction period, the results indicate that Lianjia's DBI initially prolonged the transaction period. However, this effect reversed in 2020, albeit not continuously. This is likely due to the combined effects of online consolidation and the pandemic, with initial improvements followed by subsequent deterioration. For price concessions, we find that the Lianjia's DBI is significantly negatively correlated with the price concessions during pandemic periods. This is due to the fact that most transactions slow down during these periods and people are more likely to wait longer to find a buyer, which would result in fewer price concessions.

